Deep learning models for representing out-of-vocabulary words

Communication has become increasingly dynamic with the popularization of social networks and applications that allow people to express themselves and communicate instantly. In this scenario, distributed representation models have their quality impacted by new words that appear frequently or that are derived from spelling errors. These words that are unknown by the models, known as out-of-vocabulary (OOV) words, need to be properly handled to not degrade the quality of the natural language processing (NLP) applications, which depend on the appropriate vector representation of the texts. To better understand this problem and finding the best techniques to handle OOV words, in this study, we present a comprehensive performance evaluation of deep learning models for representing OOV words. We performed an intrinsic evaluation using a benchmark dataset and an extrinsic evaluation using different NLP tasks: text categorization, named entity recognition, and part-of-speech tagging. Although the results indicated that the best technique for handling OOV words is different for each task, Comick, a deep learning method that infers the embedding based on the context and the morphological structure of the OOV word, obtained promising results.

==> includes/tab_NER_POS_fastText.tex <==
\begin{table}[!htb]
	\centering
	\scriptsize
	\caption{Performance on NER and POS tagging.}
	\label{tab:results_ner_POSTagging}
	\begin{tabular}{llcccc}
		\toprule
		
& & \multicolumn{2}{c}{NER (F-measure)} & POS tagging (accuracy) & \multirow{2}{*}{\makecell{Avg. \\ranking}} \\ \cmidrule(lr){3-4} \cmidrule(lr){5-5} 
& & Bio-NER & Rare-NER & Twitter-POS \\ \cmidrule(lr){3-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} 

\multirow{5}{*}{\rotatebox{90}{Baselines}} & FastText                               & \cellcolor{gray!60}\textbf{0.671} & \cellcolor{gray!60}\textbf{0.451} & \cellcolor{gray!60}\textbf{0.760} & \textbf{1.00} \\

& Average                                & \cellcolor{gray!46}0.627          & \cellcolor{gray!49}0.437          & \cellcolor{gray!49}0.743   & 4.33      \\

& Random                                 & \cellcolor{gray!49}0.632          & \cellcolor{gray!53}0.440          & \cellcolor{gray!32}0.738   & 5.33       \\

& Sum                                    & \cellcolor{gray!39}0.597          & \cellcolor{gray!32}0.421          & \cellcolor{gray!53}0.744      & 6.33    \\

& Zero                                   & \cellcolor{gray!53}0.635          & \cellcolor{gray!15}0.355          & \cellcolor{gray!46}0.742   & 7.50       \\ \cmidrule(lr){3-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6}

\multirow{9}{*}{\rotatebox{90}{Deep learning}} & LSTM                                   & \cellcolor{gray!35}0.593          & \cellcolor{gray!56}0.444          & \cellcolor{gray!25}0.723     & 7.00     \\

& HiCE                                   & \cellcolor{gray!32}0.589          & \cellcolor{gray!39}0.426          & \cellcolor{gray!46}0.742     & 7.17    \\

& Comick                                 & \cellcolor{gray!42}0.618          & \cellcolor{gray!42}0.431          & \cellcolor{gray!28}0.737      & 7.33    \\ 




& RoBERTa                                & \cellcolor{gray!56}0.637          & \cellcolor{gray!25}0.409          & \cellcolor{gray!18}0.716     & 8.67     \\


& DistilBERT                             & \cellcolor{gray!21}0.581          & \cellcolor{gray!18}0.387          & \cellcolor{gray!56}0.748       & 9.00   \\

& GPT2                                   & \cellcolor{gray!28}0.584          & \cellcolor{gray!46}0.436          & \cellcolor{gray!21}0.717     & 9.00     \\

& Transformer                            & \cellcolor{gray!15}0.579          & \cellcolor{gray!35}0.424          & \cellcolor{gray!39}0.741     & 9.50      \\


& Electra                                & \cellcolor{gray!25}0.583          & \cellcolor{gray!21}0.394          & \cellcolor{gray!35}0.739     & 10.33     \\

& HiCE (context)                         & \cellcolor{gray!15}0.579          & \cellcolor{gray!28}0.413          & \cellcolor{gray!15}0.704      & 12.50   \\ \midrule

	\end{tabular}
\end{table}

==> includes/tab_NER_PosTagging_estatisticas.tex <==
\begin{table}[!htb]
	\centering
	\scriptsize
	\caption{Estatísticas das OOVs nas bases de dados de NER e POS \textit{tagging}.}\label{tab:estatisticas_OOV_NER_PosTagging}
	\setlength{\tabcolsep}{2.0pt} % Default value: 6pt %margem que separa as colunas

\begin{tabular}{c|lccc} 

\toprule

\multicolumn{1}{c}{} &  & Bio-NER & Rare-NER & Twitter-POS \\ \midrule 
\multicolumn{1}{c}{} & \% of docs with OOV & 85.0 & 69.0 & 85.0 \\ \midrule 

\multirow{9}{*}{\rotatebox{90}{\makecell{\% of docs treated \\by the models}}} 
& Comick                                 & 100.0          & 100.0          & 100.0          \\
& HiCE                                   & 100.0          & 100.0          & 100.0          \\
& HiCE (context)                         & 100.0          & 100.0          & 100.0          \\

& GPT2                                   & 98.0          & 92.0          & 90.0          \\

& LSTM                                   & 98.0          & 91.0          & 89.0          \\
& Transformer                            & 98.0          & 91.0          & 89.0          \\

& DistilBERT                             & 99.0          & 84.0          & 85.0          \\

& Electra                                & 93.0          & 82.0          & 85.0          \\

& RoBERTa                                & 23.0          & 67.0          & 74.0          \\
 \midrule
	\end{tabular}
\end{table}



==> includes/tab_fastText_avg_trainSize0.7_offline_0UnknownWords_todosNiveis_analiseIndividual.tex <==
\begin{table*}
\centering
\scriptsize
\setlength{\tabcolsep}{2.0pt} % Default value: 6pt %margem que separa as colunas
\renewcommand*{\arraystretch}{0.7}
\caption{Macro F-measure  obtained  on text categorization.}%
    \label{tab:results_twitter}

	\begin{tabular}{lccccccccc}
		\toprule
 & Archeage & HCR & Hobbit & IPhone6 & OMD & SS-Tweet & STS-Test & Sanders & UMICH \\ \hline 

Zero                                   & \cellcolor{gray!53}0.846          & \cellcolor{gray!42}0.691          & \cellcolor{gray!53}0.896          & \cellcolor{gray!35}0.706          & \cellcolor{gray!18}0.773          & \cellcolor{gray!56}0.800          & \cellcolor{gray!42}0.926          & \cellcolor{gray!53}0.853          & \cellcolor{gray!53}0.958          \\
Random                                 & \cellcolor{gray!46}0.842          & \cellcolor{gray!21}0.667          & \cellcolor{gray!35}0.882          & \cellcolor{gray!28}0.703          & \cellcolor{gray!53}0.796          & \cellcolor{gray!28}0.768          & \cellcolor{gray!42}0.926          & \cellcolor{gray!35}0.842          & \cellcolor{gray!49}0.955          \\
Sum                                    & \cellcolor{gray!49}0.844          & \cellcolor{gray!49}0.700          & \cellcolor{gray!15}0.806          & \cellcolor{gray!39}0.712          & \cellcolor{gray!53}0.796          & \cellcolor{gray!21}0.763          & \cellcolor{gray!28}0.900          & \cellcolor{gray!60}\textbf{0.855} & \cellcolor{gray!39}0.946          \\
Average                                & \cellcolor{gray!32}0.829          & \cellcolor{gray!32}0.677          & \cellcolor{gray!39}0.884          & \cellcolor{gray!15}0.670          & \cellcolor{gray!21}0.775          & \cellcolor{gray!18}0.750          & \cellcolor{gray!42}0.926          & \cellcolor{gray!25}0.833          & \cellcolor{gray!39}0.946          \\
FastText                               & \cellcolor{gray!56}0.852          & \cellcolor{gray!15}0.659          & \cellcolor{gray!46}0.890          & \cellcolor{gray!25}0.700          & \cellcolor{gray!25}0.777          & \cellcolor{gray!42}0.778          & \cellcolor{gray!53}0.935          & \cellcolor{gray!39}0.845          & \cellcolor{gray!15}0.937          \\
LSTM                                   & \cellcolor{gray!32}0.829          & \cellcolor{gray!39}0.688          & \cellcolor{gray!28}0.870          & \cellcolor{gray!46}0.714          & \cellcolor{gray!32}0.782          & \cellcolor{gray!60}\textbf{0.805} & \cellcolor{gray!32}0.910          & \cellcolor{gray!32}0.839          & \cellcolor{gray!25}0.942          \\
Transformer                            & \cellcolor{gray!42}0.837          & \cellcolor{gray!28}0.671          & \cellcolor{gray!56}0.914          & \cellcolor{gray!60}\textbf{0.729} & \cellcolor{gray!46}0.789          & \cellcolor{gray!15}0.744          & \cellcolor{gray!56}0.936          & \cellcolor{gray!46}0.848          & \cellcolor{gray!39}0.946          \\
GPT2                                   & \cellcolor{gray!15}0.820          & \cellcolor{gray!53}0.703          & \cellcolor{gray!60}\textbf{0.925} & \cellcolor{gray!53}0.717          & \cellcolor{gray!32}0.782          & \cellcolor{gray!49}0.787          & \cellcolor{gray!15}0.885          & \cellcolor{gray!28}0.838          & \cellcolor{gray!46}0.952          \\
RoBERTa                                & \cellcolor{gray!25}0.828          & \cellcolor{gray!25}0.668          & \cellcolor{gray!21}0.860          & \cellcolor{gray!56}0.728          & \cellcolor{gray!60}\textbf{0.804} & \cellcolor{gray!46}0.786          & \cellcolor{gray!49}0.927          & \cellcolor{gray!18}0.821          & \cellcolor{gray!60}\textbf{0.967} \\
DistilBERT                             & \cellcolor{gray!21}0.826          & \cellcolor{gray!35}0.685          & \cellcolor{gray!42}0.888          & \cellcolor{gray!49}0.715          & \cellcolor{gray!15}0.772          & \cellcolor{gray!39}0.773          & \cellcolor{gray!18}0.891          & \cellcolor{gray!15}0.815          & \cellcolor{gray!18}0.941          \\
Electra                                & \cellcolor{gray!35}0.833          & \cellcolor{gray!56}0.707          & \cellcolor{gray!25}0.866          & \cellcolor{gray!18}0.688          & \cellcolor{gray!32}0.782          & \cellcolor{gray!39}0.773          & \cellcolor{gray!21}0.893          & \cellcolor{gray!53}0.853          & \cellcolor{gray!18}0.941          \\
HiCE                                   & \cellcolor{gray!39}0.834          & \cellcolor{gray!60}\textbf{0.712} & \cellcolor{gray!32}0.873          & \cellcolor{gray!32}0.705          & \cellcolor{gray!49}0.792          & \cellcolor{gray!53}0.789          & \cellcolor{gray!60}\textbf{0.946} & \cellcolor{gray!49}0.852          & \cellcolor{gray!28}0.943          \\
HiCE (context)                         & \cellcolor{gray!18}0.825          & \cellcolor{gray!18}0.663          & \cellcolor{gray!18}0.816          & \cellcolor{gray!21}0.696          & \cellcolor{gray!32}0.782          & \cellcolor{gray!25}0.765          & \cellcolor{gray!25}0.898          & \cellcolor{gray!18}0.821          & \cellcolor{gray!39}0.946          \\
Comick                                 & \cellcolor{gray!60}\textbf{0.853} & \cellcolor{gray!46}0.692          & \cellcolor{gray!49}0.893          & \cellcolor{gray!46}0.714          & \cellcolor{gray!42}0.783          & \cellcolor{gray!32}0.770          & \cellcolor{gray!35}0.917          & \cellcolor{gray!46}0.848          & \cellcolor{gray!56}0.964          \\ \hline

	\end{tabular}
\end{table*}


==> includes/tab_fastText_avg_trainSize0.7_offline_0UnknownWords_todosNiveis_analiseIndividual_2.tex <==
\begin{table*}
\centering
\scriptsize
\setlength{\tabcolsep}{0.5pt} % Default value: 6pt %margem que separa as colunas
%\renewcommand*{\arraystretch}{0.7}
\caption{Macro F-measure  obtained  on text categorization.}%
    \label{tab:results_twitter}

	\begin{tabular}{lcccccccccc}
		\toprule

 & \multicolumn{9}{c}{Macro F-measure} & \multirow{2}{*}{\makecell{Avg. \\ranking}} \\ \cmidrule(lr){2-10} 
 & Archeage & HCR & Hobbit & IPhone6 & OMD & SS-Tweet & STS-Test & Sanders & UMICH & \\ \cmidrule(lr){2-10}  \cmidrule(lr){11-11}

Comick                                 & \cellcolor{gray!60}\textbf{0.853} & \cellcolor{gray!46}0.692          & \cellcolor{gray!49}0.893          & \cellcolor{gray!46}0.714          & \cellcolor{gray!42}0.783          & \cellcolor{gray!32}0.770          & \cellcolor{gray!35}0.917          & \cellcolor{gray!46}0.848          & \cellcolor{gray!56}0.964          & 5.11 \\

Zero                                   & \cellcolor{gray!53}0.846          & \cellcolor{gray!42}0.691          & \cellcolor{gray!53}0.896          & \cellcolor{gray!35}0.706          & \cellcolor{gray!18}0.773          & \cellcolor{gray!56}0.800          & \cellcolor{gray!42}0.926          & \cellcolor{gray!53}0.853          & \cellcolor{gray!53}0.958          & 5.17 \\

HiCE                                   & \cellcolor{gray!39}0.834          & \cellcolor{gray!60}\textbf{0.712} & \cellcolor{gray!32}0.873          & \cellcolor{gray!32}0.705          & \cellcolor{gray!49}0.792          & \cellcolor{gray!53}0.789          & \cellcolor{gray!60}\textbf{0.946} & \cellcolor{gray!49}0.852          & \cellcolor{gray!28}0.943          & 5.33 \\

Transformer                            & \cellcolor{gray!42}0.837          & \cellcolor{gray!28}0.671          & \cellcolor{gray!56}0.914          & \cellcolor{gray!60}\textbf{0.729} & \cellcolor{gray!46}0.789          & \cellcolor{gray!15}0.744          & \cellcolor{gray!56}0.936          & \cellcolor{gray!46}0.848          & \cellcolor{gray!39}0.946          & 5.89 \\

RoBERTa                                & \cellcolor{gray!25}0.828          & \cellcolor{gray!25}0.668          & \cellcolor{gray!21}0.860          & \cellcolor{gray!56}0.728          & \cellcolor{gray!60}\textbf{0.804} & \cellcolor{gray!46}0.786          & \cellcolor{gray!49}0.927          & \cellcolor{gray!18}0.821          & \cellcolor{gray!60}\textbf{0.967} & 6.61 \\

Sum                                    & \cellcolor{gray!49}0.844          & \cellcolor{gray!49}0.700          & \cellcolor{gray!15}0.806          & \cellcolor{gray!39}0.712          & \cellcolor{gray!53}0.796          & \cellcolor{gray!21}0.763          & \cellcolor{gray!28}0.900          & \cellcolor{gray!60}\textbf{0.855} & \cellcolor{gray!39}0.946          & 6.89 \\


GPT2                                   & \cellcolor{gray!15}0.820          & \cellcolor{gray!53}0.703          & \cellcolor{gray!60}\textbf{0.925} & \cellcolor{gray!53}0.717          & \cellcolor{gray!32}0.782          & \cellcolor{gray!49}0.787          & \cellcolor{gray!15}0.885          & \cellcolor{gray!28}0.838          & \cellcolor{gray!46}0.952          & 6.94 \\


Random                                 & \cellcolor{gray!46}0.842          & \cellcolor{gray!21}0.667          & \cellcolor{gray!35}0.882          & \cellcolor{gray!28}0.703          & \cellcolor{gray!53}0.796          & \cellcolor{gray!28}0.768          & \cellcolor{gray!42}0.926          & \cellcolor{gray!35}0.842          & \cellcolor{gray!49}0.955          & 7.28 \\


LSTM                                   & \cellcolor{gray!32}0.829          & \cellcolor{gray!39}0.688          & \cellcolor{gray!28}0.870          & \cellcolor{gray!46}0.714          & \cellcolor{gray!32}0.782          & \cellcolor{gray!60}\textbf{0.805} & \cellcolor{gray!32}0.910          & \cellcolor{gray!32}0.839          & \cellcolor{gray!25}0.942          & 7.83 \\

FastText                               & \cellcolor{gray!56}0.852          & \cellcolor{gray!15}0.659          & \cellcolor{gray!46}0.890          & \cellcolor{gray!25}0.700          & \cellcolor{gray!25}0.777          & \cellcolor{gray!42}0.778          & \cellcolor{gray!53}0.935          & \cellcolor{gray!39}0.845          & \cellcolor{gray!15}0.937          & 8.11 \\

Electra                                & \cellcolor{gray!35}0.833          & \cellcolor{gray!56}0.707          & \cellcolor{gray!25}0.866          & \cellcolor{gray!18}0.688          & \cellcolor{gray!32}0.782          & \cellcolor{gray!39}0.773          & \cellcolor{gray!21}0.893          & \cellcolor{gray!53}0.853          & \cellcolor{gray!18}0.941          & 8.56 \\

Average                                & \cellcolor{gray!32}0.829          & \cellcolor{gray!32}0.677          & \cellcolor{gray!39}0.884          & \cellcolor{gray!15}0.670          & \cellcolor{gray!21}0.775          & \cellcolor{gray!18}0.750          & \cellcolor{gray!42}0.926          & \cellcolor{gray!25}0.833          & \cellcolor{gray!39}0.946          & 9.89 \\

DistilBERT                             & \cellcolor{gray!21}0.826          & \cellcolor{gray!35}0.685          & \cellcolor{gray!42}0.888          & \cellcolor{gray!49}0.715          & \cellcolor{gray!15}0.772          & \cellcolor{gray!39}0.773          & \cellcolor{gray!18}0.891          & \cellcolor{gray!15}0.815          & \cellcolor{gray!18}0.941          & 10.11 \\


HiCE (context)                         & \cellcolor{gray!18}0.825          & \cellcolor{gray!18}0.663          & \cellcolor{gray!18}0.816          & \cellcolor{gray!21}0.696          & \cellcolor{gray!32}0.782          & \cellcolor{gray!25}0.765          & \cellcolor{gray!25}0.898          & \cellcolor{gray!18}0.821          & \cellcolor{gray!39}0.946          & 11.28 \\
 \midrule

	\end{tabular}
\end{table*}


==> includes/tab_fastText_avg_trainSize0.7_offline_0UnknownWords_todosNiveis_analiseIndividual_3.tex <==
\begin{table}[!htb]
\centering
\scriptsize
\setlength{\tabcolsep}{0.5pt} % Default value: 6pt %margem que separa as colunas
%\renewcommand*{\arraystretch}{0.7}
\caption{Macro F-measure  obtained  on text categorization.}%
    \label{tab:results_twitter}

	\begin{tabular}{llcccccccccc}
		\toprule

& & \multicolumn{9}{c}{Macro F-measure} & \multirow{2}{*}{\makecell{Avg. \\ranking}} \\ \cmidrule(lr){3-11} 
& & Archeage & HCR & Hobbit & IPhone6 & OMD & SS-Tweet & STS-Test & Sanders & UMICH & \\  \cmidrule(lr){3-11}  \cmidrule(lr){12-12}

\multirow{5}{*}{\rotatebox{90}{Baselines}} & Zero                                   & \cellcolor{gray!53}0.846          & \cellcolor{gray!42}0.691          & \cellcolor{gray!53}0.896          & \cellcolor{gray!35}0.706          & \cellcolor{gray!18}0.773          & \cellcolor{gray!56}0.800          & \cellcolor{gray!42}0.926          & \cellcolor{gray!53}0.853          & \cellcolor{gray!53}0.958          & 5.17 \\

&  Sum                                    & \cellcolor{gray!49}0.844          & \cellcolor{gray!49}0.700          & \cellcolor{gray!15}0.806          & \cellcolor{gray!39}0.712          & \cellcolor{gray!53}0.796          & \cellcolor{gray!21}0.763          & \cellcolor{gray!28}0.900          & \cellcolor{gray!60}\textbf{0.855} & \cellcolor{gray!39}0.946          & 6.89 \\

&  Random                                 & \cellcolor{gray!46}0.842          & \cellcolor{gray!21}0.667          & \cellcolor{gray!35}0.882          & \cellcolor{gray!28}0.703          & \cellcolor{gray!53}0.796          & \cellcolor{gray!28}0.768          & \cellcolor{gray!42}0.926          & \cellcolor{gray!35}0.842          & \cellcolor{gray!49}0.955          & 7.28 \\

&  FastText                               & \cellcolor{gray!56}0.852          & \cellcolor{gray!15}0.659          & \cellcolor{gray!46}0.890          & \cellcolor{gray!25}0.700          & \cellcolor{gray!25}0.777          & \cellcolor{gray!42}0.778          & \cellcolor{gray!53}0.935          & \cellcolor{gray!39}0.845          & \cellcolor{gray!15}0.937          & 8.11 \\

&  Average                                & \cellcolor{gray!32}0.829          & \cellcolor{gray!32}0.677          & \cellcolor{gray!39}0.884          & \cellcolor{gray!15}0.670          & \cellcolor{gray!21}0.775          & \cellcolor{gray!18}0.750          & \cellcolor{gray!42}0.926          & \cellcolor{gray!25}0.833          & \cellcolor{gray!39}0.946          & 9.89 \\  \cmidrule(lr){3-11}  \cmidrule(lr){12-12}


\multirow{9}{*}{\rotatebox{90}{Deep learning}} & Comick                                 & \cellcolor{gray!60}\textbf{0.853} & \cellcolor{gray!46}0.692          & \cellcolor{gray!49}0.893          & \cellcolor{gray!46}0.714          & \cellcolor{gray!42}0.783          & \cellcolor{gray!32}0.770          & \cellcolor{gray!35}0.917          & \cellcolor{gray!46}0.848          & \cellcolor{gray!56}0.964          & \textbf{5.11} \\

& HiCE                                   & \cellcolor{gray!39}0.834          & \cellcolor{gray!60}\textbf{0.712} & \cellcolor{gray!32}0.873          & \cellcolor{gray!32}0.705          & \cellcolor{gray!49}0.792          & \cellcolor{gray!53}0.789          & \cellcolor{gray!60}\textbf{0.946} & \cellcolor{gray!49}0.852          & \cellcolor{gray!28}0.943          & 5.33 \\

&  Transformer                            & \cellcolor{gray!42}0.837          & \cellcolor{gray!28}0.671          & \cellcolor{gray!56}0.914          & \cellcolor{gray!60}\textbf{0.729} & \cellcolor{gray!46}0.789          & \cellcolor{gray!15}0.744          & \cellcolor{gray!56}0.936          & \cellcolor{gray!46}0.848          & \cellcolor{gray!39}0.946          & 5.89 \\

&  RoBERTa                                & \cellcolor{gray!25}0.828          & \cellcolor{gray!25}0.668          & \cellcolor{gray!21}0.860          & \cellcolor{gray!56}0.728          & \cellcolor{gray!60}\textbf{0.804} & \cellcolor{gray!46}0.786          & \cellcolor{gray!49}0.927          & \cellcolor{gray!18}0.821          & \cellcolor{gray!60}\textbf{0.967} & 6.61 \\



&  GPT2                                   & \cellcolor{gray!15}0.820          & \cellcolor{gray!53}0.703          & \cellcolor{gray!60}\textbf{0.925} & \cellcolor{gray!53}0.717          & \cellcolor{gray!32}0.782          & \cellcolor{gray!49}0.787          & \cellcolor{gray!15}0.885          & \cellcolor{gray!28}0.838          & \cellcolor{gray!46}0.952          & 6.94 \\





&  LSTM                                   & \cellcolor{gray!32}0.829          & \cellcolor{gray!39}0.688          & \cellcolor{gray!28}0.870          & \cellcolor{gray!46}0.714          & \cellcolor{gray!32}0.782          & \cellcolor{gray!60}\textbf{0.805} & \cellcolor{gray!32}0.910          & \cellcolor{gray!32}0.839          & \cellcolor{gray!25}0.942          & 7.83 \\

&  Electra                                & \cellcolor{gray!35}0.833          & \cellcolor{gray!56}0.707          & \cellcolor{gray!25}0.866          & \cellcolor{gray!18}0.688          & \cellcolor{gray!32}0.782          & \cellcolor{gray!39}0.773          & \cellcolor{gray!21}0.893          & \cellcolor{gray!53}0.853          & \cellcolor{gray!18}0.941          & 8.56 \\

& DistilBERT                             & \cellcolor{gray!21}0.826          & \cellcolor{gray!35}0.685          & \cellcolor{gray!42}0.888          & \cellcolor{gray!49}0.715          & \cellcolor{gray!15}0.772          & \cellcolor{gray!39}0.773          & \cellcolor{gray!18}0.891          & \cellcolor{gray!15}0.815          & \cellcolor{gray!18}0.941          & 10.11 \\


& HiCE (context)                         & \cellcolor{gray!18}0.825          & \cellcolor{gray!18}0.663          & \cellcolor{gray!18}0.816          & \cellcolor{gray!21}0.696          & \cellcolor{gray!32}0.782          & \cellcolor{gray!25}0.765          & \cellcolor{gray!25}0.898          & \cellcolor{gray!18}0.821          & \cellcolor{gray!39}0.946          & 11.28 \\
 \midrule

	\end{tabular}
\end{table}


==> includes/tab_fastText_avg_trainSize0.7_offline_0UnknownWords_todosNiveis_analiseIndividual_3_1artificialOOVs.tex <==
\begin{table}[!htb]
\centering
\scriptsize
\setlength{\tabcolsep}{0.5pt} % Default value: 6pt %margem que separa as colunas
%\renewcommand*{\arraystretch}{0.7}
\caption{Experiments with one artificial OOV in each message.}%
    \label{tab:results_stat_twitter_1artificialOOVs}

\subtable[][\label{tab:results_twitter_1ArtificialOOV}Macro F-measure  obtained  on text categorization.]{
	\begin{tabular}{llcccccccccc}
		\toprule

& & \multicolumn{9}{c}{Macro F-measure} & \multirow{2}{*}{\makecell{Avg. \\ranking}} \\ \cmidrule(lr){3-11} 
& & Archeage & HCR & Hobbit & IPhone6 & OMD & SS-Tweet & STS-Test & Sanders & UMICH & \\  \cmidrule(lr){3-11}  \cmidrule(lr){12-12}

\multirow{5}{*}{\rotatebox{90}{Baselines}}  & Random                                       & \cellcolor{gray!42}0.837                     & \cellcolor{gray!46}0.682                     & \cellcolor{gray!42}0.832                     & \cellcolor{gray!28}0.699                     & \cellcolor{gray!42}0.769                     & \cellcolor{gray!55}0.791                     & \cellcolor{gray!55}0.908                     & \cellcolor{gray!60}\textbf{0.844}            & \cellcolor{gray!37}0.875                     & 4.17          \\
 & Sum                                          & \cellcolor{gray!37}0.832                     & \cellcolor{gray!15}0.646                     & \cellcolor{gray!46}0.839                     & \cellcolor{gray!37}0.716                     & \cellcolor{gray!37}0.767                     & \cellcolor{gray!60}\textbf{0.806}            & \cellcolor{gray!51}0.907                     & \cellcolor{gray!28}0.811                     & \cellcolor{gray!28}0.861                     & 5.89          \\
 & Average                                      & \cellcolor{gray!33}0.831                     & \cellcolor{gray!33}0.674                     & \cellcolor{gray!24}0.804                     & \cellcolor{gray!19}0.682                     & \cellcolor{gray!46}0.773                     & \cellcolor{gray!46}0.784                     & \cellcolor{gray!33}0.872                     & \cellcolor{gray!33}0.813                     & \cellcolor{gray!55}0.891                     & 6.33          \\
 & Zero                                         & \cellcolor{gray!46}0.838                     & \cellcolor{gray!24}0.667                     & \cellcolor{gray!51}0.843                     & \cellcolor{gray!33}0.715                     & \cellcolor{gray!28}0.763                     & \cellcolor{gray!19}0.750                     & \cellcolor{gray!15}0.852                     & \cellcolor{gray!46}0.833                     & \cellcolor{gray!46}0.880                     & 6.56          
 \\  \cmidrule(lr){3-11}  \cmidrule(lr){12-12}


\multirow{9}{*}{\rotatebox{90}{Deep learning}}   & GPT2                                         & \cellcolor{gray!28}0.820                     & \cellcolor{gray!51}0.696                     & \cellcolor{gray!19}0.802                     & \cellcolor{gray!15}0.681                     & \cellcolor{gray!55}0.776                     & \cellcolor{gray!51}0.790                     & \cellcolor{gray!60}\textbf{0.930}            & \cellcolor{gray!15}0.799                     & \cellcolor{gray!60}\textbf{0.894}            & 5.61          \\
 & LSTM                                         & \cellcolor{gray!15}0.804                     & \cellcolor{gray!28}0.672                     & \cellcolor{gray!37}0.824                     & \cellcolor{gray!46}0.723                     & \cellcolor{gray!60}\textbf{0.785}            & \cellcolor{gray!42}0.775                     & \cellcolor{gray!15}0.852                     & \cellcolor{gray!42}0.822                     & \cellcolor{gray!51}0.883                     & 5.83          \\
 & DistilBERT                                   & \cellcolor{gray!51}0.840                     & \cellcolor{gray!37}0.679                     & \cellcolor{gray!60}\textbf{0.862}            & \cellcolor{gray!24}0.693                     & \cellcolor{gray!55}0.776                     & \cellcolor{gray!28}0.766                     & \cellcolor{gray!42}0.889                     & \cellcolor{gray!19}0.805                     & \cellcolor{gray!19}0.851                     & 5.94          \\
 & RoBERTa                                      & \cellcolor{gray!60}\textbf{0.847}            & \cellcolor{gray!60}\textbf{0.701}            & \cellcolor{gray!15}0.800                     & \cellcolor{gray!55}0.732                     & \cellcolor{gray!15}0.745                     & \cellcolor{gray!24}0.757                     & \cellcolor{gray!37}0.887                     & \cellcolor{gray!37}0.816                     & \cellcolor{gray!24}0.855                     & 6.22          \\
 & HiCE (context)                               & \cellcolor{gray!24}0.818                     & \cellcolor{gray!19}0.653                     & \cellcolor{gray!28}0.817                     & \cellcolor{gray!46}0.723                     & \cellcolor{gray!33}0.765                     & \cellcolor{gray!28}0.766                     & \cellcolor{gray!46}0.900                     & \cellcolor{gray!55}0.839                     & \cellcolor{gray!37}0.875                     & 6.28          \\
 & Transformer                                  & \cellcolor{gray!55}0.843                     & \cellcolor{gray!42}0.681                     & \cellcolor{gray!33}0.819                     & \cellcolor{gray!60}\textbf{0.758}            & \cellcolor{gray!24}0.762                     & \cellcolor{gray!15}0.743                     & \cellcolor{gray!28}0.861                     & \cellcolor{gray!51}0.836                     & \cellcolor{gray!15}0.780                     & 6.33          \\
 & Electra                                      & \cellcolor{gray!19}0.817                     & \cellcolor{gray!55}0.699                     & \cellcolor{gray!55}0.845                     & \cellcolor{gray!42}0.717                     & \cellcolor{gray!19}0.757                     & \cellcolor{gray!37}0.767                     & \cellcolor{gray!15}0.852                     & \cellcolor{gray!19}0.805                     & \cellcolor{gray!33}0.868                     & 6.83          \\
 \midrule

	\end{tabular}
}
\subtable[][\label{tab:results_twitter_1ArtificialOOV_stat}Statistics of the OOVs.]{
\begin{tabular}{c|m{1.9cm}ccccccccc} 

\toprule

\multicolumn{1}{c}{} &  & Archeage & HCR & Hobbit & IPhone6 & OMD & SS-Tweet & STS-Test & Sanders & UMICH \\ \midrule 

\multirow{9}{*}{\rotatebox{90}{\makecell{\% of docs \\treated by \\the models}}} 

& HiCE (context)                         & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          \\

& Electra                                & 99.0          & 99.0          & 100.0          & 100.0          & 97.0          & 99.0          & 99.0          & 99.0          & 100.0          \\

& LSTM                                   & 94.0          & 95.0          & 91.0          & 93.0          & 95.0          & 94.0          & 92.0          & 95.0          & 93.0          \\
& GPT2                                   & 94.0          & 95.0          & 91.0          & 93.0          & 95.0          & 94.0          & 92.0          & 95.0          & 93.0          \\
& Transformer                            & 94.0          & 95.0          & 91.0          & 93.0          & 95.0          & 94.0          & 92.0          & 95.0          & 93.0          \\
& DistilBERT                             & 83.0          & 69.0          & 90.0          & 85.0          & 80.0          & 87.0          & 87.0          & 76.0          & 85.0          \\
& RoBERTa                                & 19.0          & 19.0          & 15.0          & 18.0          & 24.0          & 17.0          & 20.0          & 21.0          & 23.0          \\


 \midrule



	\end{tabular}}
\end{table}


==> includes/tab_fastText_avg_trainSize0.7_offline_0UnknownWords_todosNiveis_analiseIndividual_3_2artificialOOVs.tex <==
\begin{table}[!htb]
\centering
\scriptsize
\setlength{\tabcolsep}{0.5pt} % Default value: 6pt %margem que separa as colunas
%\renewcommand*{\arraystretch}{0.7}
\caption{Experiments with two artificial OOVs in each message.}%
    \label{tab:results_stat_twitter_2artificialOOVs}

\subtable[][\label{tab:results_twitter_2ArtificialOOV}Macro F-measure  obtained  on text categorization.]{
	\begin{tabular}{llcccccccccc}
		\toprule

& & \multicolumn{9}{c}{Macro F-measure} & \multirow{2}{*}{\makecell{Avg. \\ranking}} \\ \cmidrule(lr){3-11} 
& & Archeage & HCR & Hobbit & IPhone6 & OMD & SS-Tweet & STS-Test & Sanders & UMICH & \\  \cmidrule(lr){3-11}  \cmidrule(lr){12-12}

\multirow{5}{*}{\rotatebox{90}{Baselines}}   & Average                                      & \cellcolor{gray!55}0.830                     & \cellcolor{gray!28}0.654                     & \cellcolor{gray!46}0.786                     & \cellcolor{gray!46}0.691                     & \cellcolor{gray!51}0.750                     & \cellcolor{gray!55}0.776                     & \cellcolor{gray!60}\textbf{0.872}            & \cellcolor{gray!55}0.821                     & \cellcolor{gray!60}\textbf{0.840}            & 3.06          \\
 & Zero                                         & \cellcolor{gray!33}0.821                     & \cellcolor{gray!33}0.657                     & \cellcolor{gray!15}0.704                     & \cellcolor{gray!60}\textbf{0.700}            & \cellcolor{gray!37}0.746                     & \cellcolor{gray!42}0.764                     & \cellcolor{gray!55}0.854                     & \cellcolor{gray!60}\textbf{0.824}            & \cellcolor{gray!51}0.829                     & 4.72          \\
 & Sum                                          & \cellcolor{gray!37}0.822                     & \cellcolor{gray!55}0.695                     & \cellcolor{gray!55}0.789                     & \cellcolor{gray!37}0.680                     & \cellcolor{gray!15}0.717                     & \cellcolor{gray!60}\textbf{0.779}            & \cellcolor{gray!15}0.789                     & \cellcolor{gray!28}0.796                     & \cellcolor{gray!37}0.813                     & 5.94          \\
 & Random                                       & \cellcolor{gray!46}0.825                     & \cellcolor{gray!46}0.682                     & \cellcolor{gray!24}0.732                     & \cellcolor{gray!37}0.680                     & \cellcolor{gray!24}0.728                     & \cellcolor{gray!15}0.354                     & \cellcolor{gray!42}0.827                     & \cellcolor{gray!24}0.790                     & \cellcolor{gray!28}0.806                     & 7.28          
 \\  \cmidrule(lr){3-11}  \cmidrule(lr){12-12}


\multirow{9}{*}{\rotatebox{90}{Deep learning}}    & Transformer                                  & \cellcolor{gray!19}0.810                     & \cellcolor{gray!42}0.679                     & \cellcolor{gray!46}0.786                     & \cellcolor{gray!42}0.685                     & \cellcolor{gray!55}0.758                     & \cellcolor{gray!37}0.761                     & \cellcolor{gray!37}0.825                     & \cellcolor{gray!37}0.800                     & \cellcolor{gray!60}\textbf{0.840}            & 5.00          \\
 & RoBERTa                                      & \cellcolor{gray!42}0.823                     & \cellcolor{gray!51}0.687                     & \cellcolor{gray!37}0.773                     & \cellcolor{gray!28}0.677                     & \cellcolor{gray!60}\textbf{0.760}            & \cellcolor{gray!46}0.765                     & \cellcolor{gray!24}0.815                     & \cellcolor{gray!15}0.780                     & \cellcolor{gray!46}0.818                     & 5.72          \\
 & LSTM                                         & \cellcolor{gray!51}0.829                     & \cellcolor{gray!37}0.662                     & \cellcolor{gray!28}0.756                     & \cellcolor{gray!51}0.692                     & \cellcolor{gray!46}0.747                     & \cellcolor{gray!19}0.724                     & \cellcolor{gray!51}0.852                     & \cellcolor{gray!19}0.787                     & \cellcolor{gray!33}0.812                     & 6.00          \\
 & DistilBERT                                   & \cellcolor{gray!24}0.818                     & \cellcolor{gray!15}0.641                     & \cellcolor{gray!42}0.775                     & \cellcolor{gray!55}0.699                     & \cellcolor{gray!19}0.720                     & \cellcolor{gray!51}0.766                     & \cellcolor{gray!28}0.819                     & \cellcolor{gray!51}0.815                     & \cellcolor{gray!24}0.804                     & 6.61          \\
 & Electra                                      & \cellcolor{gray!28}0.819                     & \cellcolor{gray!15}0.641                     & \cellcolor{gray!60}\textbf{0.803}            & \cellcolor{gray!19}0.676                     & \cellcolor{gray!33}0.739                     & \cellcolor{gray!33}0.759                     & \cellcolor{gray!19}0.808                     & \cellcolor{gray!46}0.814                     & \cellcolor{gray!46}0.818                     & 6.83          \\
 & GPT2                                         & \cellcolor{gray!60}\textbf{0.834}            & \cellcolor{gray!28}0.654                     & \cellcolor{gray!33}0.767                     & \cellcolor{gray!19}0.676                     & \cellcolor{gray!28}0.733                     & \cellcolor{gray!28}0.756                     & \cellcolor{gray!46}0.828                     & \cellcolor{gray!33}0.798                     & \cellcolor{gray!15}0.792                     & 7.11          \\
 & HiCE (context)                               & \cellcolor{gray!15}0.763                     & \cellcolor{gray!60}\textbf{0.702}            & \cellcolor{gray!19}0.710                     & \cellcolor{gray!15}0.666                     & \cellcolor{gray!37}0.746                     & \cellcolor{gray!24}0.749                     & \cellcolor{gray!33}0.821                     & \cellcolor{gray!42}0.806                     & \cellcolor{gray!19}0.803                     & 7.72          \\
 \midrule

	\end{tabular}
}
\subtable[][\label{tab:results_twitter_2ArtificialOOV_stat}Statistics of the OOVs.]{
\begin{tabular}{c|m{1.9cm}ccccccccc} 

\toprule

\multicolumn{1}{c}{} &  & Archeage & HCR & Hobbit & IPhone6 & OMD & SS-Tweet & STS-Test & Sanders & UMICH \\ \midrule 

\multirow{9}{*}{\rotatebox{90}{\makecell{\% of docs \\treated by \\the models}}} 

& HiCE (context)                         & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          \\

& Electra                                & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 99.0          & 100.0          & 99.0          \\

& GPT2                                   & 99.0          & 100.0          & 99.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          \\


& LSTM                                   & 98.0          & 99.0          & 99.0          & 98.0          & 100.0          & 99.0          & 99.0          & 100.0          & 97.0          \\
& Transformer                            & 98.0          & 99.0          & 99.0          & 98.0          & 100.0          & 99.0          & 99.0          & 100.0          & 97.0          \\
& DistilBERT                             & 95.0          & 86.0          & 97.0          & 92.0          & 89.0          & 93.0          & 93.0          & 86.0          & 83.0          \\
& RoBERTa                                & 35.0          & 40.0          & 34.0          & 36.0          & 48.0          & 34.0          & 38.0          & 43.0          & 49.0          \\


\midrule



	\end{tabular}}
\end{table}


==> includes/tab_fastText_avg_trainSize0.7_offline_0UnknownWords_todosNiveis_analiseIndividual_3_3artificialOOVs.tex <==
\begin{table}[!htb]
\centering
\scriptsize
\setlength{\tabcolsep}{0.5pt} % Default value: 6pt %margem que separa as colunas
%\renewcommand*{\arraystretch}{0.7}
\caption{Experiments with three artificial OOV in each message.}%
    \label{tab:results_stat_twitter_3artificialOOVs}

\subtable[][\label{tab:results_twitter_3ArtificialOOV}Macro F-measure  obtained  on text categorization.]{
	\begin{tabular}{llcccccccccc}
		\toprule

& & \multicolumn{9}{c}{Macro F-measure} & \multirow{2}{*}{\makecell{Avg. \\ranking}} \\ \cmidrule(lr){3-11} 
& & Archeage & HCR & Hobbit & IPhone6 & OMD & SS-Tweet & STS-Test & Sanders & UMICH & \\  \cmidrule(lr){3-11}  \cmidrule(lr){12-12}

\multirow{5}{*}{\rotatebox{90}{Baselines}}   & Sum                                          & \cellcolor{gray!60}\textbf{0.802}            & \cellcolor{gray!46}0.683                     & \cellcolor{gray!55}0.810                     & \cellcolor{gray!60}\textbf{0.734}            & \cellcolor{gray!46}0.706                     & \cellcolor{gray!55}0.759                     & \cellcolor{gray!42}0.856                     & \cellcolor{gray!55}0.802                     & \cellcolor{gray!60}\textbf{0.783}            & 2.44          \\
 & Average                                      & \cellcolor{gray!42}0.796                     & \cellcolor{gray!19}0.641                     & \cellcolor{gray!24}0.765                     & \cellcolor{gray!55}0.727                     & \cellcolor{gray!55}0.716                     & \cellcolor{gray!60}\textbf{0.772}            & \cellcolor{gray!55}0.881                     & \cellcolor{gray!37}0.784                     & \cellcolor{gray!15}0.672                     & 5.33          \\
 & Random                                       & \cellcolor{gray!37}0.780                     & \cellcolor{gray!51}0.692                     & \cellcolor{gray!42}0.786                     & \cellcolor{gray!37}0.721                     & \cellcolor{gray!33}0.700                     & \cellcolor{gray!46}0.757                     & \cellcolor{gray!51}0.871                     & \cellcolor{gray!19}0.746                     & \cellcolor{gray!28}0.752                     & 5.67          \\
 & Zero                                         & \cellcolor{gray!55}0.800                     & \cellcolor{gray!55}0.702                     & \cellcolor{gray!19}0.745                     & \cellcolor{gray!24}0.695                     & \cellcolor{gray!51}0.708                     & \cellcolor{gray!15}0.731                     & \cellcolor{gray!46}0.862                     & \cellcolor{gray!33}0.775                     & \cellcolor{gray!46}0.767                     & 5.72          
         
 \\  \cmidrule(lr){3-11}  \cmidrule(lr){12-12}


 & DistilBERT                                   & \cellcolor{gray!51}0.799                     & \cellcolor{gray!37}0.670                     & \cellcolor{gray!42}0.786                     & \cellcolor{gray!46}0.724                     & \cellcolor{gray!24}0.692                     & \cellcolor{gray!37}0.747                     & \cellcolor{gray!24}0.815                     & \cellcolor{gray!60}\textbf{0.821}            & \cellcolor{gray!37}0.758                     & 5.39          \\
 & RoBERTa                                      & \cellcolor{gray!24}0.766                     & \cellcolor{gray!24}0.646                     & \cellcolor{gray!60}\textbf{0.854}            & \cellcolor{gray!37}0.721                     & \cellcolor{gray!60}\textbf{0.724}            & \cellcolor{gray!24}0.737                     & \cellcolor{gray!28}0.816                     & \cellcolor{gray!51}0.799                     & \cellcolor{gray!42}0.764                     & 5.61          \\
 & Electra                                      & \cellcolor{gray!46}0.797                     & \cellcolor{gray!15}0.625                     & \cellcolor{gray!51}0.801                     & \cellcolor{gray!33}0.705                     & \cellcolor{gray!28}0.697                     & \cellcolor{gray!33}0.739                     & \cellcolor{gray!33}0.841                     & \cellcolor{gray!46}0.792                     & \cellcolor{gray!37}0.758                     & 6.44          \\
 & LSTM                                         & \cellcolor{gray!28}0.770                     & \cellcolor{gray!33}0.668                     & \cellcolor{gray!28}0.773                     & \cellcolor{gray!46}0.724                     & \cellcolor{gray!37}0.705                     & \cellcolor{gray!28}0.738                     & \cellcolor{gray!60}\textbf{0.885}            & \cellcolor{gray!15}0.729                     & \cellcolor{gray!19}0.724                     & 6.89          \\
 & HiCE (context)                               & \cellcolor{gray!33}0.773                     & \cellcolor{gray!60}\textbf{0.711}            & \cellcolor{gray!33}0.774                     & \cellcolor{gray!19}0.679                     & \cellcolor{gray!15}0.676                     & \cellcolor{gray!19}0.732                     & \cellcolor{gray!37}0.843                     & \cellcolor{gray!24}0.759                     & \cellcolor{gray!46}0.767                     & 7.17          \\
 & GPT2                                         & \cellcolor{gray!15}0.730                     & \cellcolor{gray!42}0.671                     & \cellcolor{gray!42}0.786                     & \cellcolor{gray!28}0.698                     & \cellcolor{gray!37}0.705                     & \cellcolor{gray!37}0.747                     & \cellcolor{gray!19}0.781                     & \cellcolor{gray!28}0.771                     & \cellcolor{gray!24}0.730                     & 7.44          \\
 & Transformer                                  & \cellcolor{gray!19}0.751                     & \cellcolor{gray!28}0.661                     & \cellcolor{gray!15}0.246                     & \cellcolor{gray!15}0.661                     & \cellcolor{gray!19}0.691                     & \cellcolor{gray!46}0.757                     & \cellcolor{gray!15}0.698                     & \cellcolor{gray!46}0.792                     & \cellcolor{gray!55}0.780                     & 7.89          \\
 \midrule

	\end{tabular}
}
\subtable[][\label{tab:results_twitter_3ArtificialOOV_stat}Statistics of the OOVs.]{
\begin{tabular}{c|m{1.9cm}ccccccccc} 

\toprule

\multicolumn{1}{c}{} &  & Archeage & HCR & Hobbit & IPhone6 & OMD & SS-Tweet & STS-Test & Sanders & UMICH \\ \midrule 

\multirow{9}{*}{\rotatebox{90}{\makecell{\% of docs \\treated by \\the models}}} 

& Electra                                & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          \\

& HiCE (context)                         & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          \\

& GPT2                                   & 99.0          & 100.0          & 99.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          \\

& LSTM                                   & 99.0          & 100.0          & 99.0          & 99.0          & 100.0          & 99.0          & 99.0          & 100.0          & 97.0          \\
& Transformer                            & 99.0          & 100.0          & 99.0          & 99.0          & 100.0          & 99.0          & 99.0          & 100.0          & 97.0          \\
& DistilBERT                             & 96.0          & 93.0          & 99.0          & 95.0          & 93.0          & 96.0          & 96.0          & 92.0          & 88.0          \\
& RoBERTa                                & 50.0          & 58.0          & 48.0          & 52.0          & 66.0          & 51.0          & 56.0          & 60.0          & 66.0          \\



 \midrule



	\end{tabular}}
\end{table}


==> includes/tab_fastText_avg_trainSize0.7_offline_0UnknownWords_todosNiveis_analiseIndividual_stat.tex <==
\begin{table}
\centering
\scriptsize
\setlength{\tabcolsep}{1.0pt} % Default value: 6pt %margem que separa as colunas
\renewcommand*{\arraystretch}{0.7}
\caption{Statistics of OOVs in the text categorization datasets.}%
    \label{tab:results_twitter_stat}

\begin{tabular}{c|m{1.9cm}ccccccccc} 

\toprule

\multicolumn{1}{c}{} &  & Archeage & HCR & Hobbit & IPhone6 & OMD & SS-Tweet & STS-Test & Sanders & UMICH \\ \midrule 
\multicolumn{1}{c}{} & \% of docs with OOV & 51.0 & 4.0 & 6.0 & 61.0 & 3.0 & 5.0 & 3.0 & 9.0 & 2.0 \\ \midrule 

\multirow{9}{*}{\rotatebox{90}{\makecell{\% of docs \\treated by \\the models}}} & 

 HiCE                                   & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          \\
& HiCE (context)                         & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          \\
& Comick                                 & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          \\

& Electra                                & 99.0          & 100.0          & 100.0          & 100.0          & 100.0          & 95.0          & 90.0          & 100.0          & 95.0          \\

& GPT2                                   & 91.0          & 97.0          & 93.0          & 95.0          & 88.0          & 93.0          & 90.0          & 93.0          & 79.0          \\

& LSTM                                   & 91.0          & 97.0          & 93.0          & 94.0          & 88.0          & 92.0          & 90.0          & 93.0          & 79.0          \\
& Transformer                            & 91.0          & 97.0          & 93.0          & 94.0          & 88.0          & 92.0          & 90.0          & 93.0          & 79.0          \\

& DistilBERT                             & 75.0          & 45.0          & 76.0          & 89.0          & 75.0          & 65.0          & 80.0          & 70.0          & 79.0          \\
& RoBERTa                                & 27.0          & 43.0          & 34.0          & 17.0          & 39.0          & 33.0          & 20.0          & 39.0          & 47.0          \\



 \midrule



	\end{tabular}


\end{table}


==> includes/tab_fastText_avg_trainSize0.7_offline_chimeras.tex <==
\begin{table}
\centering
\scriptsize
\setlength{\tabcolsep}{1.0pt} % Default value: 6pt %margem que separa as colunas
\renewcommand*{\arraystretch}{0.7}
\caption{Chimera - média das correlações de Spearman.}%
    \label{tab:results_fastText_offline_0UnknownWords_todosNiveis}	

\begin{tabular}{c|ccc cccccHHccHH}
		\toprule
		
	N. contexts	& Oracle & \begin{turn}{45}Average\end{turn} & Sum & \begin{turn}{45}LSTM\end{turn}  & \begin{turn}{45}Transformer\end{turn} & GPT2 & RoBERTa & DBERT & DBERTT7 & DBERTTuning & Electra & Hice & HiceContext & Comick\\ \midrule
		
		
		
2                  & \cellcolor{gray!60}\textbf{0.422} & \cellcolor{gray!49}0.279          & \cellcolor{gray!53}0.285          & \cellcolor{gray!25}0.065          & \cellcolor{gray!21}0.045          & \cellcolor{gray!35}0.158          & \cellcolor{gray!18}0.022          & \cellcolor{gray!56}0.287          & \cellcolor{gray!32}0.144          & \cellcolor{gray!46}0.214          & \cellcolor{gray!28}0.079          & \cellcolor{gray!42}0.200          & \cellcolor{gray!39}0.183          & \cellcolor{gray!15}-0.081          \\ 
4                & \cellcolor{gray!60}\textbf{0.423} & \cellcolor{gray!53}0.306          & \cellcolor{gray!49}0.300          & \cellcolor{gray!25}0.110          & \cellcolor{gray!21}0.049          & \cellcolor{gray!35}0.236          & \cellcolor{gray!18}0.028          & \cellcolor{gray!56}0.318          & \cellcolor{gray!32}0.194          & \cellcolor{gray!46}0.291          & \cellcolor{gray!28}0.170          & \cellcolor{gray!39}0.251          & \cellcolor{gray!42}0.272          & \cellcolor{gray!15}-0.099          \\ 
6                 & \cellcolor{gray!60}\textbf{0.436} & \cellcolor{gray!49}0.304          & \cellcolor{gray!46}0.301          & \cellcolor{gray!21}0.109          & \cellcolor{gray!25}0.112          & \cellcolor{gray!32}0.221          & \cellcolor{gray!18}0.032          & \cellcolor{gray!56}0.376          & \cellcolor{gray!35}0.229          & \cellcolor{gray!53}0.342          & \cellcolor{gray!28}0.172          & \cellcolor{gray!39}0.290          & \cellcolor{gray!46}0.301          & \cellcolor{gray!15}-0.068          \\  \hline

		
		
		
		\hline	
	\end{tabular}
	
\end{table}


==> includes/tab_fastText_avg_trainSize0.7_offline_chimeras_2.tex <==
\begin{table}[!htb]
\centering
\scriptsize
\setlength{\tabcolsep}{2.0pt} % Default value: 6pt %margem que separa as colunas
\renewcommand*{\arraystretch}{1.2}
\caption{Average Spearman correlation on the Chimera dataset.}%
    \label{tab:results_chimera}	

\begin{tabular}{C{0.5cm}lcccc} 

\toprule

&  & \multicolumn{3}{c}{Avg. Spearman correlation} & \multirow{3}{*}{\makecell{Avg. \\ranking}} \\ \cmidrule(lr){3-5} 

&  & 2 sentences & 4 sentences & 6 sentences & \\ \cmidrule(lr){3-5}  \cmidrule(lr){6-6}

 & Oracle                                 & 0.422 & 0.423 & 0.436 & - - \\ \cmidrule(lr){3-5} \cmidrule(lr){6-6}

%\multicolumn{6}{c}{} \\
\multirow{2}{*}{\rotatebox{90}{\makecell{Base-\\lines}}} 
%\multirow{2}{*}{\rotatebox{90}{\makecell{Base-\\lines}}}
& Average                                & \cellcolor{gray!45}0.279          & \cellcolor{gray!50}0.306          & \cellcolor{gray!50}0.304          & 2.33 \\
& Sum                                    & \cellcolor{gray!50}0.285          & \cellcolor{gray!45}0.300          & \cellcolor{gray!40}0.301          & 2.83 \\ 
%\multicolumn{6}{c}{} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-6} 

\multirow{7}{*}{\rotatebox{90}{\makecell{Deep\\learning}}} & DistilBERT                             & \cellcolor{gray!55}\textbf{0.287}          & \cellcolor{gray!55}\textbf{0.318}         & \cellcolor{gray!55}\textbf{0.376}          & \textbf{1.00} \\

& HiCE (context)                         & \cellcolor{gray!40}0.183          & \cellcolor{gray!40}0.272          & \cellcolor{gray!40}0.301         & 3.83 \\

& GPT2                                   & \cellcolor{gray!35}0.158          & \cellcolor{gray!35}0.236          & \cellcolor{gray!35}0.221           & 5.00 \\


& Electra                                & \cellcolor{gray!30}0.079          & \cellcolor{gray!30}0.170          & \cellcolor{gray!30}0.172         & 6.00  \\

& LSTM                                   & \cellcolor{gray!25}0.065          & \cellcolor{gray!25}0.110          & \cellcolor{gray!20}0.109          & 7.33 \\
& Transformer                            & \cellcolor{gray!20}0.045          & \cellcolor{gray!20}0.049          & \cellcolor{gray!25}0.112           & 7.67 \\

& RoBERTa                                & \cellcolor{gray!15}0.022          & \cellcolor{gray!15}0.028          & \cellcolor{gray!15}0.032          & 9.00 \\

 \midrule

	\end{tabular}
	
\end{table}


==> includes/tab_fastText_avg_trainSize0.7_offline_chimeras_3.tex <==
\begin{table}[!htb]
\centering
\scriptsize
\setlength{\tabcolsep}{6.0pt} % Default value: 6pt %margem que separa as colunas
\renewcommand*{\arraystretch}{0.7}
\caption{Average Spearman correlation on the Chimera dataset.}%
    \label{tab:results_chimera}	

\begin{tabular}{lcccc} 

\toprule

 & \multicolumn{3}{c}{Avg. Spearman correlation} & \multirow{3}{*}{\makecell{Avg. \\ranking}} \\ \cmidrule(lr){2-4} 

 & 2 sentences & 4 sentences & 6 sentences & \\ \cmidrule(lr){2-4}  \cmidrule(lr){5-5}

Oracle                                 & 0.422 & 0.423 & 0.436 &  \\ \cmidrule(lr){2-4} 

DistilBERT                             & \cellcolor{gray!55}\textbf{0.287}          & \cellcolor{gray!55}\textbf{0.318}         & \cellcolor{gray!55}\textbf{0.376}          & 1.00 \\

Average                                & \cellcolor{gray!45}0.279          & \cellcolor{gray!50}0.306          & \cellcolor{gray!50}0.304          & 2.33 \\
Sum                                    & \cellcolor{gray!50}0.285          & \cellcolor{gray!45}0.300          & \cellcolor{gray!40}0.301          & 2.83 \\

HiCE (context)                         & \cellcolor{gray!40}0.183          & \cellcolor{gray!40}0.272          & \cellcolor{gray!40}0.301         & 3.83 \\

GPT2                                   & \cellcolor{gray!35}0.158          & \cellcolor{gray!35}0.236          & \cellcolor{gray!35}0.221           & 5.00 \\


Electra                                & \cellcolor{gray!30}0.079          & \cellcolor{gray!30}0.170          & \cellcolor{gray!30}0.172         & 6.00  \\

LSTM                                   & \cellcolor{gray!25}0.065          & \cellcolor{gray!25}0.110          & \cellcolor{gray!20}0.109          & 7.33 \\
Transformer                            & \cellcolor{gray!20}0.045          & \cellcolor{gray!20}0.049          & \cellcolor{gray!25}0.112           & 7.67 \\

RoBERTa                                & \cellcolor{gray!15}0.022          & \cellcolor{gray!15}0.028          & \cellcolor{gray!15}0.032          & 9.00 \\

 \midrule

	\end{tabular}
	
\end{table}


==> includes/tab_fastText_avg_trainSize0.7_offline_chimeras_stat.tex <==
\begin{table}
\centering
\scriptsize
\setlength{\tabcolsep}{2.0pt} % Default value: 6pt %margem que separa as colunas
\renewcommand*{\arraystretch}{0.7}
\caption{Estatísticas - Chimeras.}%
    \label{tab:results_fastText_offline_0UnknownWords_todosNiveis}

\begin{tabular}{l|C{1.5cm}|cc ccccccccc}
	\hline

N. contexts    & \% Doc. com OOVs & \multicolumn{10}{c}{\% de Doc. tratados} \\ 		
     & & LSTM  & Transformer & GPT2 & RoBERTa & DBERT & DBERTT7 & DBERTTuning & Electra  & Hice & HiceContext & Comick \\ \hline

2                 & 100.0 & 97.0          & 97.0          & 97.0          & 9.0          & 95.0          & 99.0          & 98.0          & 100.0          & 100.0          & 100.0          & 100.0          \\ 
4                 & 100.0 & 97.0          & 97.0          & 97.0          & 10.0          & 95.0          & 99.0          & 98.0          & 99.0          & 100.0          & 100.0          & 100.0          \\ 
6                 & 100.0 & 97.0          & 97.0          & 97.0          & 10.0          & 95.0          & 99.0          & 98.0          & 99.0          & 100.0          & 100.0          & 100.0          \\  \hline

	\end{tabular}	
\end{table}


==> includes/tab_fastText_avg_trainSize0.7_offline_chimeras_stat_2.tex <==
\begin{table}[!htb]
\centering
\scriptsize
\setlength{\tabcolsep}{2.0pt} % Default value: 6pt %margem que separa as colunas
\renewcommand*{\arraystretch}{0.7}
\caption{Percentage of OOVs treated by the deep learning models.}%
    \label{tab:results_chimeras_stat}

\begin{tabular}{lccc}
\toprule

 & 2 sentences & 4 sentences & 6 sentences \\ \midrule 

HiCE (context)                         & 100.0          & 100.0          & 100.0          \\ 
Electra                                & 100.0          & 99.0          & 99.0          \\
LSTM                                   & 97.0          & 97.0          & 97.0          \\
Transformer                            & 97.0          & 97.0          & 97.0          \\
GPT2                                   & 97.0          & 97.0          & 97.0          \\
DistilBERT                             & 95.0          & 95.0          & 95.0          \\
RoBERTa                                & 9.0          & 10.0          & 10.0          \\
\midrule

	\end{tabular}	
\end{table}


==> includes/tab_textosFormais_fastText_avg_trainSize0.7_offline_0UnknownWords_analiseIndividual.tex <==
\begin{table}[!htb]
\centering
\scriptsize
\setlength{\tabcolsep}{3.5pt} % Default value: 6pt %margem que separa as colunas
\renewcommand*{\arraystretch}{0.95}
\caption{Experiments on text categorization -- formal texts.}%
    \label{tab:results_statistics_formalTexts}

\subtable[][\label{tab:results_formalTexts}Macro F-measure  obtained  on text categorization.]{
	\begin{tabular}{llcccccccc} 
		\toprule

& & \multicolumn{6}{c}{Macro F-measure} & \multirow{2}{*}{\makecell{Avg. \\ranking}} \\ \cmidrule(lr){3-8} 
& & 7sectors          & Amazon          & IMDB          & Yelp          & Ohsumed          & Reuters-21578 & \\  \cmidrule(lr){3-8}  \cmidrule(lr){9-9}

\multirow{5}{*}{\rotatebox{90}{Baselines}} 

 & FastText                                     & \cellcolor{gray!49}0.970                     & \cellcolor{gray!25}0.830                     & \cellcolor{gray!35}0.797                     & \cellcolor{gray!28}0.840                     & \cellcolor{gray!60}\textbf{0.287}            & \cellcolor{gray!53}0.928                     & 6.25          \\
 & Random                                       & \cellcolor{gray!56}0.971                     & \cellcolor{gray!53}0.854                     & \cellcolor{gray!15}0.767                     & \cellcolor{gray!42}0.851                     & \cellcolor{gray!28}0.277                     & \cellcolor{gray!42}0.920                     & 6.83          \\
 & Zero                                         & \cellcolor{gray!15}0.949                     & \cellcolor{gray!42}0.845                     & \cellcolor{gray!49}0.822                     & \cellcolor{gray!42}0.851                     & \cellcolor{gray!46}0.283                     & \cellcolor{gray!21}0.889                     & 7.67          \\
 & Average                                      & \cellcolor{gray!21}0.958                     & \cellcolor{gray!60}\textbf{0.877}            & \cellcolor{gray!28}0.791                     & \cellcolor{gray!18}0.825                     & \cellcolor{gray!49}0.284                     & \cellcolor{gray!32}0.912                     & 8.17          \\
 & Sum                                          & \cellcolor{gray!28}0.962                     & \cellcolor{gray!18}0.820                     & \cellcolor{gray!32}0.794                     & \cellcolor{gray!25}0.831                     & \cellcolor{gray!21}0.276                     & \cellcolor{gray!49}0.924                     & 10.00          \\
  \cmidrule(lr){8-8}


\multirow{9}{*}{\rotatebox{90}{Deep learning}}                          

 & Electra                                      & \cellcolor{gray!60}\textbf{0.973}            & \cellcolor{gray!28}0.838                     & \cellcolor{gray!60}\textbf{0.824}            & \cellcolor{gray!60}\textbf{0.867}            & \cellcolor{gray!28}0.277                     & \cellcolor{gray!39}0.918                     & 5.00          \\
 & RoBERTa                                      & \cellcolor{gray!56}0.971                     & \cellcolor{gray!28}0.838                     & \cellcolor{gray!49}0.822                     & \cellcolor{gray!32}0.841                     & \cellcolor{gray!56}0.285                     & \cellcolor{gray!46}0.921                     & 5.33          \\
 & Transformer                                  & \cellcolor{gray!35}0.968                     & \cellcolor{gray!35}0.842                     & \cellcolor{gray!46}0.815                     & \cellcolor{gray!53}0.859                     & \cellcolor{gray!56}0.285                     & \cellcolor{gray!28}0.906                     & 6.08          \\
 & HiCE (context)                               & \cellcolor{gray!35}0.968                     & \cellcolor{gray!56}0.855                     & \cellcolor{gray!18}0.782                     & \cellcolor{gray!35}0.844                     & \cellcolor{gray!21}0.276                     & \cellcolor{gray!56}0.930                     & 7.42          \\
 & Comick                                       & \cellcolor{gray!28}0.962                     & \cellcolor{gray!49}0.853                     & \cellcolor{gray!39}0.806                     & \cellcolor{gray!15}0.820                     & \cellcolor{gray!28}0.277                     & \cellcolor{gray!60}\textbf{0.934}            & 7.75          \\
 & DistilBERT                                   & \cellcolor{gray!42}0.969                     & \cellcolor{gray!46}0.848                     & \cellcolor{gray!21}0.788                     & \cellcolor{gray!56}0.862                     & \cellcolor{gray!15}0.274                     & \cellcolor{gray!28}0.906                     & 8.17          \\
 & LSTM                                         & \cellcolor{gray!32}0.963                     & \cellcolor{gray!15}0.813                     & \cellcolor{gray!60}\textbf{0.824}            & \cellcolor{gray!49}0.857                     & \cellcolor{gray!35}0.278                     & \cellcolor{gray!15}0.858                     & 8.33          \\
 & GPT2                                         & \cellcolor{gray!49}0.970                     & \cellcolor{gray!39}0.843                     & \cellcolor{gray!21}0.788                     & \cellcolor{gray!35}0.844                     & \cellcolor{gray!35}0.278                     & \cellcolor{gray!18}0.882                     & 8.50          \\
 & HiCE                                         & \cellcolor{gray!18}0.950                     & \cellcolor{gray!21}0.823                     & \cellcolor{gray!42}0.811                     & \cellcolor{gray!21}0.828                     & \cellcolor{gray!42}0.280                     & \cellcolor{gray!35}0.916                     & 9.50          \\
 
 \midrule

	\end{tabular}}
\subtable[][\label{tab:results_twitter_stat}Statistics of the OOVs.]{
\begin{tabular}{c|lcccccc} 

\toprule

\multicolumn{1}{c}{} &  & 7sectors          & Amazon          & IMDB          & Yelp          & Ohsumed          & Reuters-21578 \\ \midrule 
\multicolumn{1}{c}{} & \% of docs with OOV & 91.0 & 2.0 & 2.0 & 1.0 & 79.0 & 53.0 \\ \midrule 

\multirow{9}{*}{\rotatebox{90}{\makecell{\% of docs \\treated by \\the models}}}  

& HiCE                                   & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          \\
& HiCE (context)                         & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          \\
& Comick                                 & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          & 100.0          \\ 
& Electra                                & 98.0          & 100.0          & 100.0          & 100.0          & 99.0          & 86.0          \\

& GPT2                                   & 100.0          & 100.0          & 95.0          & 91.0          & 100.0          & 98.0          \\

& LSTM                                   & 100.0          & 100.0          & 95.0          & 91.0          & 100.0          & 97.0          \\
& Transformer                            & 100.0          & 100.0          & 95.0          & 91.0          & 100.0          & 97.0          \\
& DistilBERT                             & 91.0          & 92.0          & 95.0          & 91.0          & 99.0          & 85.0          \\
& RoBERTa                                & 41.0          & 29.0          & 18.0          & 36.0          & 26.0          & 45.0          \\


 \midrule



	\end{tabular}}

\end{table}

